An Abstract Semantics of the Global View of Choreographies

We introduce an abstract semantics of the global view of choreographies. Our semantics is given in terms of pre-orders and can accommodate different lower level semantics. We discuss the adequacy of our model by considering its relation with communicating machines, that we use to formalise the local view. Interestingly, our framework seems to be more expressive than others where semantics of global views have been considered. This will be illustrated by discussing some interesting examples.

==> eptcsdata.tex <==
\providecommand{\firstpage}{67}
\providecommand{\publicationstatus}{M. Bartoletti, L. Henrio, S. Knight, and H. T. Vieira (Eds.):\\9th Interaction and Concurrency Experience (ICE 2016)\\
EPTCS 223, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.223.5}{10.4204/EPTCS.223.5}}
\pdfoutput=1

